Code to Comment "Translation": Data, Metrics, Baselining & Evaluation

The relationship of comments to code, and in particular, the task of generating useful comments given the code, has long been of interest. The earliest approaches have been based on strong syntactic theories of comment-structures, and relied on textual templates. More recently, researchers have applied deep learning methods to this task, and specifically, trainable generative translation models which are known to work very well for Natural Language translation (e.g., from German to English). We carefully examine the underlying assumption here: that the task of generating comments sufficiently resembles the task of translating between natural languages, and so similar models and evaluation metrics could be used. We analyze several recent code-comment datasets for this task: CodeNN, DeepCom, FunCom, and DocString. We compare them with WMT19, a standard dataset frequently used to train state of the art natural language translators. We found some interesting differences between the code-comment data and the WMT19 natural language data. Next, we describe and conduct some studies to calibrate BLEU (which is commonly used as a measure of comment quality). using "affinity pairs" of methods, from different projects, in the same project, in the same class, etc; Our study suggests that the current performance on some datasets might need to be improved substantially. We also argue that fairly naive information retrieval (IR) methods do well enough at this task to be considered a reasonable baseline. Finally, we make some suggestions on how our findings might be used in future research in this area.

==> includes.tex <==
\usepackage{fancybox}

\usepackage{graphicx}
\graphicspath{{figures/}}
\DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\usepackage{amsmath}
%\usepackage{floatrow}
\usepackage{subfigure}
\usepackage{caption}
\DeclareCaptionType{copyrightbox}
%\usepackage{subcaption}

\usepackage{verbatim}
\usepackage{fancyvrb}
\usepackage{color}
\usepackage{algorithmic}
\usepackage{array}
\usepackage{hyperref}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{booktabs}
\usepackage{listings}
\usepackage{eqparbox}
%\usepackage{fixltx2e}
\usepackage{stfloats}
%
\usepackage{url}
\usepackage{comment}
\usepackage{framed}
\usepackage{pdfsync}
\usepackage{ifthen}
\usepackage{balance}
% call this with optional  [turnoff] to turn off notes and todos

%\usepackage[turnon]{notes}%[turnoff]
%\usepackage{microtype}
%\usepackage{multirow}
%\usepackage[]{biblatex}
%\newtheorem{definition}{Definition}
\usepackage{xspace}


%\renewcommand{\baselinestretch}{0.97}


\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.,}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace}
\newcommand{\vs}{\hbox{\emph{v.s.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}

\newtheorem{theorem}{Theorem}[section]
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\varname}[1]{{\small\texttt{#1}}\xspace}
%\newcommand{\tom}[1]{{\color{red} Tom: #1}\xspace}
\newcommand{\ch}[1]{{\color{black} #1}\xspace}
%\newfloatcommand{capbtabbox}{table}[][\FBwidth]

\newcommand{\gh}{GitHub\xspace}

\newcommand{\C}{{\tt C}\xspace}
\newcommand{\cpp}{{\tt C++}\xspace}
\newcommand{\csharp}{{\tt C\#}\xspace}
\newcommand{\objc}{{\tt Objective-C}\xspace}
\newcommand{\go}{{\tt Go}\xspace}
\newcommand{\java}{{\tt Java}\xspace}
\newcommand{\perl}{{\tt Perl}\xspace}
\newcommand{\py}{{\tt Python}\xspace}
\newcommand{\python}{{\tt Python}\xspace}
\newcommand{\php}{{\tt Php}\xspace}
\newcommand{\ruby}{{\tt Ruby}\xspace}
\newcommand{\js}{{\tt Java\-Script}\xspace}
\newcommand{\cs}{{\tt Coffee\-Script}\xspace}
\newcommand{\ts}{{\tt Type\-Script}\xspace}
\newcommand{\clojure}{{\tt Clojure}\xspace}
\newcommand{\erlang}{{\tt Er\-lang}\xspace}
\newcommand{\haskell}{{\tt Haskell}\xspace}
\newcommand{\scala}{{\tt Scala}\xspace}

\newcommand{\FDSM}{{\tt Functional-Dynamic-Strong-Managed}\xspace} 		
\newcommand{\FSSM}{{\tt Functional-Static-Strong-Managed}\xspace}  		
\newcommand{\PSSM}{{\tt Proc-Static-Strong-Managed}\xspace}         		
\newcommand{\PSWU}{{\tt Proc-Static-Weak-Unmanaged}\xspace}         		
\newcommand{\SDSM}{{\tt Script-Dynamic-Strong-Managed}\xspace}     		
\newcommand{\SDWM}{{\tt Script-Dynamic-Weak-Managed}\xspace}        		

\newcommand{\FDSMt}{{\tt Functional\--Dynamic\--Strong\--Managed}\xspace} 		
\newcommand{\FSSMt}{{\tt Functional\--Static\--Strong\--Managed}\xspace}  		
\newcommand{\PSSMt}{{\tt Proc Static\--Strong\--Managed}\xspace}         		
\newcommand{\PSWUt}{{\tt Proc Static\--Weak\--Unmanaged}\xspace}         		
\newcommand{\SDSMt}{{\tt Script\--Dynamic\--Strong\--Managed}\xspace}     		
\newcommand{\SDWMt}{{\tt Script\--Dynamic\--Weak\--Managed}\xspace}        		

%\newcommand{\pswu}{{procedural\-\_static\-\_weak\-\_unmanaged }\xspace}
%\newcommand{\pssm}{{procedural\-\_static\-\_strong\-\_managed }\xspace}
%\newcommand{\fssm}{{functional\_static\-\_strong\_manged }\xspace}
%\newcommand{\fdsm}{{functional\_dynamic\-\_strong\_manged }\xspace}

\newcommand{\fdsm}{{\tt Functional\--Dynamic\--Strong\--Managed}\xspace} 		
\newcommand{\fssm}{{\tt Functional\--Static\--Strong\--Managed}\xspace}  		
\newcommand{\pssm}{{\tt Proc\--Static\--Strong\--Managed}\xspace}         		
\newcommand{\pswu}{{\tt Proc\--Static\--Weak\--Unmanaged}\xspace}         		
\newcommand{\sdsm}{{\tt Script\--Dynamic\--Strong\--Managed}\xspace}     		
\newcommand{\sdwm}{{\tt Script\--Dynamic\--Weak\--Managed}\xspace}        		



\newcommand{\pd}[1]{{\scriptsize \todo{Prem:  {\color{blue} #1}}}}
\newcommand{\tableshrink}[1]{\vspace{-0.25in}}


%-------------------------------------------------------------------------------------------
% Research Questions and Results
%
\newcounter{RQCounter}

 %Pass in label for rq, then rq
%

\newcommand{\RQ}[2]{%
\refstepcounter{RQCounter} \label{#1}
	\vspace{0.1in} \noindent \textbf{RQ\arabic{RQCounter}.~#2 \vspace{0.05in}}
	
}

\newcommand{\RQBoxed}[2]{%
\refstepcounter{RQCounter} \label{#1}
\begin{framed}%
\filbreak
	%\noindent\textbf{Research Question \arabic{RQCounter}: }%
	\noindent\textbf{RQ\arabic{RQCounter}: }%
#2\end{framed}
}


% Pass in label for associated research question
%
\newcommand{\RS}[2]{%
\begin{framed}%
\filbreak
	%\noindent
\textbf{Result {\ref{#1}}:~}{\emph {#2}}%
\end{framed}
}




==> notes+todos.tex <==

Remaining Experiments: 

- (David)Do a bootstrap of the BLEU for IR across splits, 
   folds done for deepcom (across projects) This is a cross-project variance experiment *medium priority*
   do folds for  CodeNN (or Docstring)  This is a truly random split variance experimetn  *medium * 
   do folds for NL de-en. with IR This gets a sense of De-En varies across random splits for NL.  *lower*
   
%- (David) add the table of  the affinity groups. TODO... Different BLEUs across affinity groups. *high priority* 
%- (David) Ensure that our BLEU calculation for the COlumbia dataset is what they do. *high priority*
%- (David) make data loader for RQ1 hybrid-deepcom *high* 
%--(David) fleshing out the  IR (how it works) *medium* 
--(David) Flesh out discussion about new columbia dataset, in 3 and 3.1 *medium*

-- Figure out how how going to address METEOR / ROGUE

(HARI) Create all violin plots (4 plots, interproj, intraproj, intraclass, SimilarAPI) *high priority, wait for David to pull the trigger, in case he does it himself* 
(HARI) Add lines for the new data to figure 1-3, and then add rows to Table 2. *high priority* 
(HARI) use the RQ1 loader above to redo the Fig1-3 plots.

- (David) Figure out CIDEr score?

Remaining Writing. 


% (prem) writea bit more on the IR section
% (prem) models etc
(prem) Threats to validity. 
 (Prem) Add discussion about standardizing evaluation with a server? 
(prem) look at the requirements for reproducibility packages. 

(Prem) move Figure 4 to top of page 6

(DEFERRED)- (David) look into how FunCom extracted comments for David's Table. 
    - Try to find FunCom's tokenization function
    - Run affinity groups with this function or a "first sentence" function



**************************************************************

Rough outline of paper

Backgound motivation: 

--study of existing datasets. For each dataset: 
    zipf plot of desired outputs
    effect of most frequent bi/trigrams on BLUE scores. 
   
---  IR performance


---how good is BLEU anyway: Inter-project, intra-class, and matched methods.

Meeting notes 3/13: (to bediscussed next week)

Hari's plots on effect of freq. ngram on BLEU were reviewed. 
we will no longer do the MUSE dataset. 
We will need to add to the paper some discussion on the confusing
arising from differences in methods used. 

TODO FOR 3/20

(following 3 questions re the frequency vs. bleu plots) 
---why does the docstring bigram look so much like the natural language plot
---why does the funcom trigram show such dramatic dropoff. 
---why is codenn trigram plot so smooth

David will get the Levenshtein filtered similar methods. 
    - Sometimes works but usually is too noisy. Next need to prototype something around most popular methods
    - Should pull the existing datsaets as a backup really soon.

Hari will get these parwise similarity plots: 

    univariate plots --one pairwise similarity histogram on comments vs. one parise similarity histogram NL. Two boxplots would be good. 
    bivariate plots --pairwise sim on inputs vs. pairwise sim on ouputs. sim using smoothed bleu
 
Prem will work on the paper.



David Notes/Todos:
    - Why does deepcom report so much better than codenn? Try to figure out if they are doing equivalent eval?
    - Do Code-nn SQL
    - Rerun the oracle bleu including NL and docstring
    - 
    
    
    
